PLATO: Pointer Learner for Agent and Task Openness

Open agent systems (OASYS) are increasingly prevalent in real-world domains where the sets of agents and tasks change unpredictably over time. Such openness, including agent openness (AO) and task openness (TO), poses a fundamental challenge to multi-agent reinforcement learning (MARL), which typically assumes fixed state and action spaces. Existing methods address openness only partially: padding and masking approaches introduce artificial bounds, while recent graph-based or hypergraph methods handle one dimension of openness but still depend on restrictive assumptions. In this paper, we introduce Pointer Learner for Agent and Task Openness (PLATO), a pointer-network-based actor combined with a centralized graph neural network (GNN) critic, trained with multi-agent proximal policy optimization under a centralized training and decentralized execution paradigm. Our pointer-based actor outputs distributions directly over the current task set. This directly supports changing action spaces without masking or retraining. Our GNN critic encodes agent-task interactions as a graph that changes shape with task and agent composition. Together, these components consider AO and TO without the boundedness of existing approaches. We formalize PLATO in a Task-and-Agent-Open Markov Game (TaAgO-MG), extending prior task-open formulations, and prove it is well-defined over the resulting unbounded state and action spaces. We evaluate PLATO with the Methods for Open Agent Systems Evaluation Initiative (MOASEI) wildfire suppression domain, an environment designed for open multi-agent system evaluation, and we demonstrate strong performance and more consistent zero-shot generalization than state-of-the-art baselines in OASYS.

==> checklist.tex <==
\section*{NeurIPS Paper Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1--2 sentence) justification right after your answer (even for \answerNA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will also be asked to include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While \answerYes{} is generally preferable to \answerNo{}, it is perfectly acceptable to answer \answerNo{} provided a proper justification is given (e.g., error bars are not reported because it would be too computationally expensive'' or ``we were unable to find the license for the dataset we used''). In general, answering \answerNo{} or \answerNA{} is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS Paper Checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}
    % \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The abstract and introduction state four contributions: (1) PLATO as the first MARL method addressing AO and TO jointly without fixed bounds or retraining, (2) the TaAgO-MG formalization with formal well-definedness and permutation-invariance proofs (Appendix~A), (3) empirical comparison against baselines across openness setups (Sections~5--6), and (4) zero-shot generalization to unseen grid sizes. All claims are directly supported by the experimental results and formal proofs presented in the paper.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A \answerNo{} or \answerNA{} answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The conclusion (Section~8) discusses three limitations: (1) the current TaAgO-MG formulation assumes one action per task, restricting application to domains requiring per-task action sets; (2) the policy assumes full observability of agents and tasks, which may not hold in practice; and (3) evaluation is confined to the MOASEI wildfire domain, leaving generalization to other open-system domains as future work.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper has no limitation while the answer \answerNo{} means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate ``Limitations'' section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We include a Lemma and Theorems outlining our proofs in the main body of the paper, with full proofs and assumptions in Appendix A.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We include extensive reproducibility details in Appendix B. This includes both the hyperparameter tuning space and the final hyper parameters for shown results.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item If the paper includes experiments, a \answerNo{} answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and\slash or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We will publish the code and reasonable documentation used to produce our experiments upon publication.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so \answerNo{} is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We describe enough of the Wildfire environment to understand the results shown in the main body of the paper. We formally define reward bounds for Wildfire in A.4, and we provide additional explanation of the domain in C.1.
    \item[] Guidelines: 
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We show the std in all tables as well as denoting Shapiro-Wilcoxon significance (with Bonferroni correction) in bold.  
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The authors should answer \answerYes{} if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g., negative error rates).
        \item If error bars are reported in tables or plots, the authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: In Appendix~B we include hardware details, hyperparameter tuning ranges, and compute estimates. Each training run takes approximately 3--5 CPU-days; the full suite (all methods, grids, setups, and tuning trials) required approximately 6{,}000--10{,}000 CPU-days in total.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We reviewed the listed guidelines, and we examined and ensured we maintain anonymity in submitted materials.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer \answerNo, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Openness work remains fairly theoretical for now, and is thus detached from societal impacts.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that there is no societal impact of the work performed.
        \item If the authors answer \answerNA{} or \answerNo, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate Deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our method has no known or anticipated risks with release.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This work uses the free-range-zoo API for its experiments. This is under the GNU3 license.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Other than the code upon publication, we do not include any additional assets.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset\slash code\slash model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our work does not include any human studies or crowd sourcing.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our work does not include any human studies or crowd sourcing. 
    \item[] Guidelines:  
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does \emph{not} impact the core methodology, scientific rigor, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our work does not involve LLMs.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy in the NeurIPS handbook for what should or should not be described.
    \end{itemize}

\end{enumerate}

==> sections/6-ablation.tex <==


% ==========================
% OVERVIEW
% ==========================

This section analyzes the encoder and pointer scoring choices in PLATO. We test four variants from a factorial design crossing two encoder choices (MLP, LSTM) with two scorer choices (additive, dot-product):  \textbf{(mlp+add)}, \textbf{(mlp+dot)}, \textbf{(lstm+add)}, and \textbf{(lstm+dot)}.  The reference design is \textbf{(mlp+add)} (Figure~\ref{fig:architecture} and Algorithm~\ref{alg:plato}). Table~\ref{tab:ablation_reward} shows the results. Additional metrics are in Appendix~\ref{sec:ablation_appendix}.



\begin{table*}[!t]
\centering
\setlength{\tabcolsep}{1.4pt}
\renewcommand{\arraystretch}{1.02}
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{\hspace{2pt}}l|r|r|r|r||r|r|r|r@{\hspace{2pt}}}
\toprule
 & \multicolumn{4}{c||}{trained and tested on $3\times3$} & \multicolumn{4}{c}{trained and tested on $4\times4$} \\
\cmidrule(lr){2-5}\cmidrule(lr){6-9}
\shortstack[l]{PLATO} & \multicolumn{1}{c|}{S0} & \multicolumn{1}{c|}{S1} & \multicolumn{1}{c|}{S2} & \multicolumn{1}{c||}{S3} & \multicolumn{1}{c|}{S0} & \multicolumn{1}{c|}{S1} & \multicolumn{1}{c|}{S2} & \multicolumn{1}{c}{S3} \\
\midrule
(mlp+add)      & 8.00$\pm$0.00 & 7.52$\pm$1.46 & 112.83$\pm$12.62 & 80.53$\pm$19.66 & 12.00$\pm$0.00 & 19.47$\pm$9.33 & 228.81$\pm$21.99 & 149.35$\pm$27.33 \\
(mlp+dot)      & 8.00$\pm$0.00 & 7.28$\pm$1.54 & 109.65$\pm$13.60 & 84.37$\pm$20.79 & 12.00$\pm$0.00 & 19.76$\pm$9.51 & 221.04$\pm$24.03 & 146.63$\pm$25.99 \\
(lstm+add)     & 8.00$\pm$0.00 & 7.47$\pm$1.36 & 108.56$\pm$14.33 & 82.12$\pm$22.23 & 12.00$\pm$0.00 & 16.12$\pm$6.75 & 227.59$\pm$24.53 & 151.33$\pm$24.35 \\
(lstm+dot)     & 8.00$\pm$0.00 & 7.20$\pm$1.61 & 113.67$\pm$15.30 & 88.16$\pm$17.87 & 12.00$\pm$0.00 & 19.49$\pm$8.57 & 218.79$\pm$23.32 & 148.31$\pm$26.50 \\
\specialrule{1.5pt}{0pt}{0pt}
 & \multicolumn{4}{c||}{trained on $2\times3$ and tested (zero-shot) on $3\times3$} & \multicolumn{4}{c}{trained on $2\times3$ and tested (zero-shot) on $4\times4$} \\
\cmidrule(lr){2-5}\cmidrule(lr){6-9}
\shortstack[l]{PLATO} & \multicolumn{1}{c|}{S0} & \multicolumn{1}{c|}{S1} & \multicolumn{1}{c|}{S2} & \multicolumn{1}{c||}{S3} & \multicolumn{1}{c|}{S0} & \multicolumn{1}{c|}{S1} & \multicolumn{1}{c|}{S2} & \multicolumn{1}{c}{S3} \\
\midrule
(mlp+add)      & 9.97$\pm$0.33  & 6.83$\pm$2.87          & 80.75$\pm$12.65 & 4.95$\pm$28.12           & 11.73$\pm$2.51          & 5.31$\pm$9.89  & 64.11$\pm$15.58 & 13.68$\pm$36.62 \\
(mlp+dot)      & 10.00$\pm$0.00 & 6.25$\pm$3.01          & 78.19$\pm$12.02 & 4.52$\pm$27.48           & \textbf{12.96$\pm$1.93} & 4.09$\pm$8.57  & 63.17$\pm$16.43 & 17.89$\pm$36.82 \\
(lstm+add)     & 9.84$\pm$0.91  & 6.52$\pm$2.64          & 71.79$\pm$22.24 & \textbf{18.49$\pm$27.48} & 11.09$\pm$2.78          & 7.37$\pm$9.37  & 66.88$\pm$11.67 & \textbf{37.97$\pm$32.54} \\
(lstm+dot)     & 9.89$\pm$0.80  & 6.31$\pm$3.39          & 82.87$\pm$16.74 & 6.19$\pm$28.53           & 10.32$\pm$2.95          & 4.56$\pm$6.30  & 65.76$\pm$18.18 & 25.56$\pm$36.38 \\
\bottomrule
\end{tabular}%
}
\caption{Ablation: Episode return (mean $\pm$ std). \textit{Top:} native evaluation; no variant achieves statistically significant best performance. \textit{Bottom:} zero-shot transfer; bold indicates statistically significant best performance. Shapiro-Wilk-adaptive two-sided test; Bonferroni-corrected, $p{<}0.0125$.}
\label{tab:ablation_reward}
\end{table*}

% ==========================
% ANALYSIS
% ==========================

\textbf{Q1: Does temporal memory in the encoder improve task selection?}
An LSTM encoder~\citep{lstm} maintains a hidden state across timesteps, while the MLP encoder is stateless and parallelizable but carries no observation history. Thus, LSTM adds sequential overhead and extra parameters.
We compare \textbf{(mlp+add) vs.\ (lstm+add)} and \textbf{(mlp+dot) vs.\ (lstm+dot)} to isolate the encoder across both scoring functions. In native evaluation, there are no statistically significant differences between LSTM and MLP variants under either scorer. In zero-shot transfer, the encoder's impact depends on the scorer and setup. With additive scoring, (lstm+add) achieves statistically significantly higher returns than (mlp+add) in S3 across both target grids (18.49 vs.\ 4.95 on $3\times3$; 37.97 vs.\ 13.68 on $4\times4$); (lstm+dot) is also numerically higher than (mlp+dot) in S3 (6.19 vs.\ 4.52 on $3\times3$; 25.56 vs.\ 17.89 on $4\times4$) but without statistical significance. %In contrast, with dot-product scoring, (mlp+dot) achieves statistically significantly higher returns than (lstm+dot) in S0 at $4\times4$ (12.96 vs.\ 10.32), indicating that temporal memory can be detrimental in simpler setups under this scorer. 
Together, these results show that the benefit of temporal memory is not universal: it is most pronounced under combined agent and task openness (S3) in zero-shot settings when paired with additive scoring.

\textbf{Q2: How does additive attention scoring perform with respect to dot-product scoring?}
Additive (Bahdanau) attention~\citep{bahdanau2014neural} scores agent-task compatibility via learned projections: $u_x^t = \mathbf{v}^\top\!\tanh(\mathbf{W}_K k_x^t + \mathbf{W}_q q^t)$, capturing asymmetric relationships at the cost of extra parameters. Dot-product scoring ($u_x^t = q^{t\top} k_x^t$) uses no extra parameters and measures similarity directly in embedding space. We compare \textbf{(mlp+add) vs.\ (mlp+dot)} and \textbf{(lstm+add) vs.\ (lstm+dot)}. In native evaluation, no scorer achieves statistically significant advantage under either encoder. In zero-shot transfer, the scorer's advantage also depends on the encoder and setup. With the LSTM encoder, (lstm+add) achieves statistically significantly higher returns than (lstm+dot) in S3 across both target grids (18.49 vs.\ 6.19 on $3\times3$; 37.97 vs.\ 25.56 on $4\times4$) — additive scoring wins in the most open zero-shot setting. With the MLP encoder, (mlp+dot) achieves statistically significantly higher returns than (mlp+add) in S0 at $4\times4$ (12.96 vs.\ 11.73) — dot-product scoring wins in the simplest zero-shot setting. %Taken together with Q1, these results point to a consistent interaction: (lstm+add) is the best combination under combined AO+TO (S3), while (mlp+dot) is the best combination under closed environment (S0) in zero-shot transfer.




%\textbf{Q3: Do team statistics improve coordination under agent openness?}
%Under AO, team composition changes dynamically; an agent unaware of its current team may redundantly target tasks covered by teammates. Team statistics (\textbf{ts}) provide a permutation-invariant summary of teammate observations, $d^t = [\mu, \mathrm{Var}, \min, \max](o_N^t) \in \mathbb{R}^{4f_N}$, at $O(|N^t|)$ cost (Appendix~\ref{app:stats-perm}). We compare \textbf{(mlp+add) vs.\ (no-team-stats)}. Dropping \textbf{ts} reduces returns in S2 across both grids, indicating a benefit under high task density. In S3, effects are genuinely mixed: at native $4\times4$ (152.56 vs.\ 149.35) and in zero-shot $4\times4$ S3 (16.83 vs.\ 13.68), (no-team-stats) matches or exceeds (mlp+add), showing no consistent coordination benefit under combined agent and task openness.

%\textbf{Q4: Where is the use of the GNN critic advantageous?}
%The GNN critic builds a bipartite agent-task graph $\mathcal{G}^t$ and runs message passing at $O(|N^t||X^t|)$ per step, with no hardcoded count bounds, enabling zero-shot transfer to larger configurations. The padded MLP critic in \textbf{(no-gnn)} zero-fills observations to training-time sizes (as in DGN~\citep{dgn} and DICG~\citep{dicg}), which hardcodes the maximum agent and task counts. We compare \textbf{(mlp+add) vs.\ (no-gnn)}. On native evaluation, both critics perform similarly. On zero-shot transfer from $2\times3$ (Table~\ref{tab:ablation_zs_reward}), (no-gnn) shows higher mean returns than (mlp+add) in S3 across both target grids (6.13 vs.\ 4.95 on $3\times3$; 21.55 vs.\ 13.68 on $4\times4$), indicating the padded MLP critic can transfer to unseen sizes when trained on small grids. Additional zero-shot results from $3\times3$ training (Appendix~\ref{sec:ablation_appendix}) show (mlp+add) outperforming (no-gnn) in S3 at $4\times4$ (57.36 vs.\ 48.05), suggesting the GNN critic's generalization advantage becomes more apparent as training grid size increases.

%\textbf{Q5: Does the pointer mechanism itself drive performance?}
%All factorial variants (Q1--Q2) retain the pointer mechanism: content-based attention producing a distribution over the current task set, with output size adapting at each step. In \textbf{(no-ptr)}, the pointer actor is replaced with a padded fixed-output MLP classifier whose output size is fixed to the training-time maximum task count. We compare \textbf{(mlp+add) vs.\ (no-ptr)}. The pointer mechanism outperforms the fixed classifier in S2 in native evaluation ($3\times3$ and $4\times4$) and in zero-shot S2 from $2\times3$ training. However, in zero-shot S3, (no-ptr) shows higher mean returns than (mlp+add) in several configurations, including $4\times4$ S3 from $2\times3$ training (29.45 vs.\ 13.68), though differences are not statistically significant owing to high variance. The pointer's advantage is most consistent in native evaluation under high task density (S2).


==> sections/junks/methodology.tex <==
%\small Overview of the PLATO architecture. The pointer actor module processes local observations into agent and task embeddings, and then selects actions through three interconnected components: (1) Agent Encoding summarizes agent composition via mean, variance, minimum, and maximum statistics ($\mathbf{stats}$), embeds them with an MLP, and propagates temporal information through a memory LSTM to yield a recurrent query; (2) Task Encoding maps task features into the latent space, conditions them on the query through a key integrator, and organizes them into a sequence processed by an LSTM encoder; and (3) the Pointer Network combines the query with the encoded task sequence using additive attention to produce logits that define a distribution over available actions. The critic module evaluates the global state as a bipartite agent–task graph, where (1) a Graph Generator builds the graph structure, (2) a Node Encoder embeds agent and task features, (3) Graph Convolutional Layers capture relational dependencies, (4) Global Pooling aggregates node embeddings into a fixed-size representation, and (5) an MLP Head outputs the centralized value estimate.}



% \textbf{task encoding} (see \ref{taskencoding}), the observed tasks at time $t$, $\mathbf{o}^t_X$, are mapped into a hidden space conditioned on the aforementioned query. We do this per task through a \emph{key integrator} so that the key of each task is aware of the context of current agents and independent of other keys. 
%%producing a sequence for the pointer mechanism (see \ref{taskencoding}). 
% We combine each key with the query  through \textbf{the pointer decoder} to form an action distribution. The decoder attends over the key sequence with an additive attention mechanism that incorporates the query into each key independently, then normalizes the result.
%%The pointer head then attends over this task sequence with an additive attention mechanism that incorporates query and key into compatibility scores, ensuring each output logit reflects both task attributes and agent context. 

% These architectural elements make the pointer actor permutation invariant, scalable to unbounded sets of agents and tasks, adaptable as agents join or leave, and capable of producing valid action distributions over any number of tasks without retraining, padding, or index manipulation.

%%We use a pointer-network based actor (which we refer to as the pointer actor) that serves as the shared policy module in PLATO, enabling consistent behavior under agent openness where new or existing agents reuse the same parameters of the learned policy without retraining.
%In detail, the pointer actor preprocesses local observations (see \ref{obs_pre}) into two sets of features that serve as inputs for the subsequent encoding steps, using two novel designs: (a) \textit{agent encoding} (see \ref{agent_query}), where the present agents at time $t$ are summarized (see \ref{a_stats}) and passed through an MLP  to have an encoded summary, then we pass the encoded summery to LSTM to form a query (see \ref{eq:qt}), and (b) \textit{task encoding} (see \ref{taskencoding}), where the available tasks at time $t$ will later be mapped into a hidden space, conditioned on the query through a key integrator (see \ref{key_integrator}), and organized into a sequence for the pointer mechanism (see \ref{taskencoding}). The pointer head then attends over this sequence to produce the action distribution.

%%Several architectural choices ensure that the pointer actor is both permutation-invariant and scalable to unbounded set sizes. First, we compute summary \textbf{agent statistics} (mean, variance, minimum, and maximum) over the features of the current agent set to produce a fixed-length representation of the agent composition at time $t$ (see~\ref{a_stats}). This summary is inherently permutation-invariant and adapts seamlessly as agents join or leave the system. Second, we feed these statistics into a recurrent \textbf{LSTM} that produces the query vector. This recurrent query carries temporal context and smooths out abrupt changes, stabilizing the policy’s decisions over time even as agents appear or disappear (mitigating volatility when there is high agent churn; see \ref{agent_query}). Third, for each available task we generate a \textbf{task embedding} and then apply a \emph{key integrator} that adds the query vector to each task’s representation (see \ref{key_integrator}). This makes each task’s encoded key \emph{aware} of the current agents’ context, and it allows the pointer mechanism to flexibly handle any number of tasks without retraining (see \ref{taskencoding}). Finally, the \textbf{pointer head} uses an additive attention mechanism that directly incorporates the agent’s query when computing compatibility scores. In other words, the pointer head’s attention logits jointly reflect each task’s attributes and the current agent context. Because each output logit corresponds to one of the current tasks (or a no-op), the pointer actor can naturally produce a valid action distribution over an arbitrary number of tasks (with no need for padding or index trickery) and is invariant to any reordering of agents or tasks in the inputs.



%TODO Position free embeding
%MLP ENCODER
%ATTENTION DECODER
%POINTER + LSTM permutation invar break TODO
%Reasoning for single step decoding pointer head
%why no multi step

%\subsubsection{\textbf{Observation Preprocessor}}\label{obs_pre}
% This component separates agent and task features, enabling each encoder to handle its respective form of openness through specialized mechanisms.
% At each timestep $t$, the environment provides agents local observations $\mathbf{O^t}=\{o^t_i\}_{i=1}^{|N|}$. The preprocessor is a deterministic function that factors $\mathbf{O}$ into two tensors for encoding: agent features $\mathbf{o}_N^t$ and task features $\mathbf{o}^t_X$. This separation of agent and task features allows the pointer actor to handle each form of openness with a specialized encoding pipeline: one for the variable agent set and one for the variable task set.




% \subsubsection{\textbf{Agent Encoding (query path)}}\label{agent_query}
% Agent encoding receives agent features from the Observation Preprocessor (see~\ref{obs_pre}), aggregates them via Agent Statistics (see~\ref{a_stats}) to obtain a permutation-invariant summary of the current agent composition, maps this summary through an MLP to project it into the latent feature space, and updates it with an LSTM to produce a temporally smoothed recurrent query $q^t$ (see Eq~\ref{eq:qt}). This query captures both the current composition and its temporal context, and is shared with the Key Integrator in Task Encoding (see~\ref{key_integrator},~\ref{taskencoding}) and the attention mechanism in the Pointer Head (see~\ref{pointer_head}) to ensure consistent agent-aware decision-making across modules.


% %Agent encoding produces a recurrent query from the current agent set by summarizing composition with set-level statistics and updating it over time with an LSTM.

% \paragraph{\textbf{Agent Statistics.}}\label{a_stats}
% To address agent openness, this component summarizes the current agent set through a novel design that computes element-wise statistics (mean, variance, minimum, maximum) over agent features. The result is a fixed-length, permutation-invariant summary of agent composition. At time $t$, the agent composition is approximated by applying  statistical functions on $\mathbf{o}^t_n$:
% \begin{equation}
% d^t
%   = \big[\;\mu(\mathbf{o}^t_N),\;\sigma^2(\mathbf{o}^t_N),\;\min(\mathbf{o}^t_N),\;\max(\mathbf{o}^t_N)\;\big], \label{eq:agent-stats}
% \end{equation}
% where $\mu$ (mean), $\sigma^2$ (variance), $\min$ (minimum), and $\max$ (maximum) are statistical functions applied across agents.  
% $d^t$, is a size-agnostic, permutation-invariant signature of agent composition at time $t$. Using multiple statistics (instead of just a mean or sum) reduces the risk of aliasing different distributions of agent features into the same summary (for example, two very different sets of agents could share the same average feature vector). We then project $d^t$ through a feedforward network (MLP) to obtain an encoded summary $e^t_N = \mathrm{MLP}_s(d^t)$.

% These statistics form the \emph{query} for our pointer network later. We create the query by encoding the Statistics with a multilayer perceptron (MLP)~\cite{rumelhart1986learning_mlp}. Then, we use a long-short term memory module \cite{lstm} to smooth our query over time,
% \begin{equation}\label{eq:qt}
% q^t = \mathrm{LSTM} \left (\mathrm{MLP}_s \left (d^t \right ), q^{t-1} \right ).
% \end{equation}

% \noindent\textit{where} \(q^t\) is the recurrent query at time \(t\);
% \(q^{t-1}\) is the previous query;
% \(\mathrm{MLP}_s(\cdot)\) is a feedforward encoder for the agent statistics \(d^t\);
% and \(\mathrm{LSTM}(\cdot)\) updates the query using the current encoded input and past hidden state.



% In effect, $q^t$ summarizes the agent set at time $t$ while incorporating knowledge of past compositions through the LSTM state $q^{t-1}$. This temporal smoothing is important for stable policy behavior: when the agent set changes unpredictably from $t-1$ to $t$ (due to agents arriving or departing), the LSTM’s memory helps $q^t$ adapt smoothly rather than changing erratically. Because the LSTM processes only the summary $e^t_N$ (which does not depend on any ordering of agents), the query $q^t$ is insensitive to the permutation of agents in $\mathbf{o}_N^t$. In other words, agent encoding produces a query that is both representative of the current agent set and consistent over time, without being tied to any particular ordering of agents.

%TODO Old content replaced by above
%where $\mathrm{MLP}_a$ is a feedforward encoder that maps the statistics vector $\mathbf{a}_s$ into a latent representation  $\mathbf{e}_s $.  
%This yields explicit \emph{awareness of the agent composition} at each step, and because the statistics depend on \textit{feature statistics rather than identities}, \emph{previously unseen agents with similar features can be captured at execution time} without retraining.

%TODO, need a distinctive name.
%\paragraph{\textbf{LSTM}}\label{agent_lstm}
%This component encodes the agent statistics with an LSTM to produce a temporally smoothed query that carries forward agents context, ensuring stable adaptation as agents enter or exit under openness. Specifically, the latent representation $\mathbf{e}_s$ is passed to an LSTM~\cite{lstm} unit:
% \begin{equation}
% \mathbf{h}_s = \mathrm{LSTM}_{\mathrm{a}}(\mathbf{e}_s),
% \end{equation}
% where $\mathrm{LSTM}_{\mathrm{a}}$ is a recurrent encoder that preserves temporal memory across timesteps. Its hidden state $\mathbf{h}_s$ serves as the recurrent \emph{query}. Encoding the agent statistics with an LSTM yields a temporally smoothed query that carries forward agents context, enabling stable adaptation under AO and TO.

%\paragraph{\textbf{Permutation Invariant Query.}}
%The LSTM maintains permutation invariance with respect to agent ordering while providing temporal consistency across timesteps. Because $\mathbf{e}_s$ is derived from permutation-invariant statistics (mean, variance, minimum, maximum) over the agent set, any reordering of agents in $\mathbf{o}_t^{(a)}$ yields identical input to the LSTM. The recurrent encoder processes a \emph{temporal sequence of composition summaries} rather than a spatial sequence of individual agents, thus preserving permutation invariance in the agent dimension while capturing temporal dependencies in the time dimension. This design ensures that the query $\mathbf{h}_s$ adapts smoothly to dynamic changes in agents composition—agents can join or leave in any order without affecting the learned representation—while the LSTM's hidden state carries forward historical context to stabilize decision-making under rapid agent churn.
 %because these statistics summarize the entire agent set, the query representation adapts smoothly as agents join or leave, enabling stable decision-making under agent openness (AO).   

%**************************************

% \subsubsection{\textbf{Task Encoding (key path)}} \label{taskencoding}

% This component encodes the current set of available tasks into latent key representations for attention-based action selection. It receives raw task features from the Observation Preprocessor (see~\ref{obs_pre}) and projects them through an MLP to obtain task embeddings. These embeddings are then conditioned on the agent’s recurrent query (see~\ref{agent_query}) via the key integrator (see~\ref{key_integrator}), producing agent-aware task keys that reflect both task attributes and agent context. The resulting integrated keys $\mathbf{k}^t$ are passed to the pointer head (see~\ref{pointer_head}), where attention computes the final action distribution over the dynamic task set.

%%The task encoding module maps raw task observations into key vectors that are compared against the agent query (see~\ref{agent_query}), enabling attention to select among variable task sets in a agent composition-aware manner.

% \paragraph{Task Encoder.}\label{task_encoder} 
% This component maps each raw task observation into a latent key embedding through an MLP, producing task representations that capture essential task attributes while remaining compatible with variable task set sizes.
% \begin{equation}
% k^{t_x} = \mathrm{MLP}_k(o^t_x), \label{eq:task-mlp}
% \end{equation}
% \noindent\textit{where} \(k^{t_x}\) is the latent key embedding for task \(x\) at time \(t\);
% \(o^t_x \in \mathbf{o}^t_X\) is the raw feature vector of task \(x\);
% \(\mathrm{MLP}_k(\cdot)\) is a feedforward encoder that maps task features to the latent space;
% and \(\mathbf{k}^t = [k^{t_1}, \ldots, k^{t_{|\mathbf{o}^t_X|}}]\) is the collection of all encoded task keys.
% We consider no-op actions through a learnable embedding projected through the same MLP and appended to $\mathbf{k}^t$.  
% This full vector of keys, $\mathbf{K}^t$, is:
% \begin{equation}
% \mathbf{K}^t = [k^t_1; \dots; k^t_{|\mathbf{o}^t_X|}; k^t_{\textsc{NOOP}}]. \label{eq:task-stack}
% \end{equation}

% \paragraph{Key Integrator.}\label{key_integrator} 

% This component conditions each task embedding on the current agents context (see~\ref{agent_query}) by integrating the agent query into task keys, yielding agent-aware representations for attention-based selection.
%%In attention, each item $i$ is represented by a \emph{key} vector $\mathbf{k}_i$ that is compared to a \emph{query} $\mathbf{q}$; a compatibility score (e.g., $u_i=\mathbf{v}^\top\tanh(\mathbf{W}_k\mathbf{k}_i+\mathbf{W}_q\mathbf{q})$) determines how much the model should focus on item $i$. In PLATO, keys are the encoded task representations that the agent’s query attends over to select an action.

% In attention mechanisms, generally, each candidate (here, a task) is represented by a \emph{key}, which interacts with a \emph{query} to compute attention scores for selection. To inject the agents' context, $q^t$, into every available task to obtain an agent-aware selection, we adopt a key-integration operation inspired by modulation-based feature fusion (e.g., FiLM \cite{perez2018film}):  
% \begin{equation}\label{eq:key-integrator-eq}
% e^t_{K,x} = \mathrm{MLP}(k^t_x + \mathbf{W}_c \times q^t), \qquad 
% \mathbf{e}^t_K = [e^t_1; \dots; e^t_{|\mathbf{o}^t_X|}; e^t_{\textsc{NOOP}}]
% \end{equation}

%% redundant.
%%Shifting task keys by the agent query makes them agent-aware, so our design of the attention scores reflects both task attributes and the current agents while preserving permutation invariance.  

%% do we need this? -NOPE
%%This operation applies the query to all available tasks in $O(|\mathbf{o}_t^{(t)}|)$ time, avoiding the $\mathcal{O}(|\mathbf{o}^t_N|\cdot|\mathbf{o}^t_X|)$ cost of explicit agent–task pairings, while preserving permutation invariance.
% \noindent\textit{where} \(e^t_{K,x}\) is the integrated key embedding for task \(x\);
% \(k^t_x\) is the encoded task key from Eq.~\eqref{eq:task-mlp};
% \(\mathbf{W}_c\) is a learnable projection matrix aligning the query dimension with task embeddings;
% \(q^t\) is the recurrent agent query from Eq.~\eqref{eq:qt};
% \(\mathrm{MLP}(\cdot)\) is a feedforward layer that fuses task and query features;
% and \(\mathbf{e}^t_K\) is the full set of agent-aware task embeddings, including the no-op key \(e^t_{\textsc{NOOP}}\).


% Note that this agent-aware conditioning, to our knowledge, has not appeared in MARL or pointer-network policies. Prior MAPPO and transformer-based methods (e.g., \cite{mappo, foerster2018counterfactual_coma, dgn, gpl, dicg}) either concatenate or cross-attend embeddings, which requires fixed structures or masking and scales as $\mathcal{O}(|N|\cdot|X|)$. In contrast, our formulation injects the agent context into each task key through a shared linear projection, producing agent-aware task embeddings in $\mathcal{O}(|X|)$ time. This explicit conditioning simplifies attention learning and improves stability under openness.

%**************************************
%\subsubsection{\textbf{Pointer Decoder}}\label{pointer_head}
%This component is a modified pointer-network decoder that transforms the agent based query and task based keys into a stochastic policy conditioned on agent composition, enabling robust action selection under openness. It uses one-step attention \cite{attention} to decode $q^t,e^t_K\to \pi$. This differs from typical pointer networks \cite{ptr}, which use an LSTM in its decoder. Next we discuss, this and other decoder changes for openness.

%Unlike the original design, which relies on an LSTM decoder with sequential processing, our pointer network %employs an MLP encoder for task keys and 
%
% by architectural modifications for openness, and consists of three key components that transform  keys $\mathbf{K}^t$ into actionable policies, as summarized below.


%\paragraph{\textbf{MLP Encoder}}\label{pointer_encoder}
%Instead of using a conventional decoder to attend over the input sequence and the hidden representation for each input element (as generated by the LSTM-based encoder), we employ an MLP encoder to ensure both \emph{permutation invariance} and \emph{position-free embeddings}. Conventional pointer networks that use LSTM decoders introduce position-dependent biases because they process tasks sequentially. The encoder processes each integrated key independently:
%\begin{equation}
%\mathbf{E}_{k,i} = \mathrm{MLP}_{\mathrm{enc}}(\mathbf{sk}_{t,i}), \quad i = 1, \ldots, |\mathbf{o}_t^{(t)}| + 1
%\end{equation}
%This position-free encoding is crucial for openness because it allows the network to reason about task relationships regardless of task ordering or set size. Tasks may have intrinsic properties that influence selection priority, and the MLP captures these features without imposing artificial sequential dependencies. By avoiding recurrent architectures at this stage, we ensure that reordering tasks in $\mathbf{sk}_t$ does not affect their learned representations.


%\paragraph{\textbf{Attention Mechanism}}


%In conventional pointer networks, the decoder is an LSTM that maintains a hidden state across steps, while attention computes compatibility scores between the decoder state (query) and the encoder outputs (keys). These scores are normalized to obtain a distribution over key positions with a support $|\text{keys}|$. 
%therefore, the attention weights themselves constitute the output rather than a fixed vocabulary. 
%TO requires us to select \emph{one task per timestep} rather than an ordered sequence (as in TSP \cite{flood1956traveling}). We already model temporal continuity in the agent encoder's LSTM (see Section~\ref{agent_query}). Requiring only one task position allows us to replace the sequential decoder with a one-step attention mechanism, which treats keys independently. This avoids position bias and better supports openness.  


%The critic (Section~\ref{critic}) constructs a bipartite agent–task graph from the global state, encodes agent and task nodes into a shared hidden space with lightweight MLPs, propagates relational information via two GCN layers with a residual connection, and aggregates by global mean pooling; a small pre-head MLP then feeds a single linear value head to produce the centralized state value.



%We present a Graph Neural Network (GNN)-based value critic for our system. Our approach leverages graph convolutions \cite{kipf2016semi} to capture relationships between agents and environmental elements (fires) in a unified representation space, enabling effective value function approximation in complex multi-agent scenarios.  This approach helps the pointer network policy to estimate the value of each open state of the environment.
%\begin{equation} \label{eq:gcn}
%\mathbf{H}^{(\ell)} = \text{ReLU}\!\left(\tilde{\mathbf{D}}^{-1/2} \tilde{\mathbf{A}} \tilde{\mathbf{D}}^{-1/2} \mathbf{H}^{(\ell-1)} \mathbf{W}^{(\ell)} \right),
%\end{equation}


%The centralized critic builds a bipartite agent–task graph (see \ref{global_graph}) from the global state (see Figure \ref{fig:global_graph}), encodes agent and task nodes with an MLP (see \ref{node_encoder}) into a shared hidden space, and propagates relational information through two GCN layers (see \ref{gcn}). We use mean pooling to aggregate node embeddings into a fixed-size representation. We pass this representation through an MLP and a final linear layer to produce the scalar state value (see \ref{critic_valuehead}). This GNN-based design \cite{kipf2016semi} captures agent-task interactions in openness, without padding or concatenation, enabling an effective value approximation in openness and providing reliable value estimates for the pointer network policy.


%We use two GCN layers to capture both direct (agent–task) and second-order (agent–task–agent/task–agent–task) interactions, while avoiding the over-smoothing issues that arise with deeper stacks. The encoded graph $\mathbf{e}_g$ is passed through two GCNs to propagate relational information among nodes. At layer $\ell$, the representation is updated as


% which is finally passed to a linear value head to estimate the state value:
% \begin{equation}
% V(s_t) = \mathbf{W}_v \mathbf{z} + b_v.
% \end{equation}

%eqref


% where . The per-update complexity is
% \begin{equation}
% M_{\mathrm{time}}^{\mathcal{L}_V}=
% \mathcal{O}\!\left(f_V \cdot (|\mathcal{N}|+|\mathcal{X}|) + |\mathcal{E}| \cdot f_V + |\mathcal{B}|\right).
% \end{equation}




%Both actor and critic parameters are optimized jointly using Adam~\cite{kingma2014adam},
%with gradient clipping and early stopping based on approximate KL divergence %\cite{kullback1997information} for stability.








%\paragraph{Convergence under Openness.}
%In conventional reinforcement learning, convergence is often determined by the stabilization of cumulative episode rewards.
%However, under openness, this criterion becomes unreliable: each episode may yield variable returns due to changing agent counts, task sets, and interaction dynamics. 
%We experimented with an alternative strategy based on monitoring policy parameter stability, i.e., measuring updates in $\theta$ or the magnitude of changes in gradients across episodes. 
%While this approaches provided a more reward-agnostic signal, it introduced two additional hyperparameters --- the magnitude threshold and the episode window size --- that proved difficult to tune reliably. 
%TODO number of episodes might change.
%For fairness and reproducibility, we therefore adopted a fixed training horizon of 500{,}000 episodes for PLATO and all baseline methods. Empirically, we observed that by this point learning curves stabilized across different configurations, providing a consistent and robust stopping criterion.




%\subsection{Training and Optimization} The model weights are initialized using orthogonal initialization with gain 0.5 to prevent the activation magnitudes from exploding as they flow through the network:
%\begin{equation}
%\initW \sim \text{Orthogonal}(0.5), \quad \initb \sim \mathcal{N}(0, 0)
%\end{equation}
%Layer normalization is applied after each encoder to stabilize learning:
%\begin{equation}
%\layernorm(\mathbf{x}) = \frac{\mathbf{x} - \mu}{\sigma} \odot \boldsymbol{\gamma} + \boldsymbol{\beta}
%\end{equation}
%where $\mu$ and $\sigma$ are computed across the feature dimension.
 %TODO hyper parameters for our solution
 %TODO Computing Hardware or setup
 %TODO PROofs & theorms
%\subsubsection{Critic Efficiency.} The critic runs in $\bigO(|\edgeset| \cdot d_h + |\nodeset| \cdot d_h^2)$ time and $\bigO(|\nodeset| \cdot d_h + |\edgeset|)$ space. We optimize memory via in-place operations, vectorized pooling.






%We employ Multi-Agent Proximal Policy Optimization (MAPPO) \cite{mappo} with Centralized Training and Decentralized Execution (CTDE) paradigm. 












%********************END of ACTOR%



%This design enables handling \emph{task openness} 
%natively: new tasks can be evaluated against the existing agents context without retraining, as attention operates in a learned feature space rather than fixed task indices.

%This should be shown as one piece later.
%In terms of complexity, the per-update time scales linearly with the number of available tasks $|\mathcal{X}|$, the policy hidden dimension, $f_\pi$, and $\mathcal{B}$:
%\begin{equation}
%M_{\mathrm{time}}^{\mathcal{L}_\pi}=\mathcal{O}\!\left(f_\pi \cdot |\mathcal{X}| + |\mathcal{B}|\right).
% \end{equation}

%and parameters are updated using the Adam optimizer \cite{kingma2014adam}.
%\subsubsection{Actor Loss} \label{actor_loss}
% \subsubsection{Critic Loss}\label{critic_loss}
%The centralized critic estimates $V_\phi(s_t)$ on the bipartite graph $\mathcal{G}^t=(\mathcal{N},\mathcal{X},\mathcal{E})$. The loss uses the PPO clipped value formulation~\cite{ppo}:%. We  describe PLATO in detail,  with the \textit{shared pointer-network actor} in Section~\ref{actor}, and the \textit{centralized GNN critic} in Section~\ref{crit}ic. 
% Finally, Algorithm~\ref{alg:plato} presents the .

%PLATO integrates pointer networks \cite{ptr} as shared actors with graph neural networks \cite{gnn} as centralized critics, trained jointly within a multi-agent proximal policy optimization framework \cite{mappo}. 


%\subsection{Differentiability}\label{sec:differentiability}
%MAPPO is a policy gradient method, it requires a differentiable policy and critic network. PLATO is differentiable with respect to its parameters $\theta$, $\phi$, and the learned no-op vector NO-OP.




%\textit{Proof.}   
%Each component of PLATO is a composition of differentiable and (subdifferentiable functions. The statistical functions in Eq.~\eqref{eq:agent-stats} (mean, variance, min, max) are piecewise-linear or smooth and admit subgradients. Each MLP consists of affine maps and ReLU or $\tanh$ activations, and are differentiable everywhere.  
%(iii) The LSTM in Eq.~\eqref{eq:qt} uses smooth gates (sigmoid, $\tanh$) and is fully differentiable.  
%(iv) The attention mechanism in Eq.~\eqref{eq:attention} is composed of affine projections, $\tanh$, and inner products, all differentiable.  
%(v) The softmax in  the policy output is smooth; gradients are computed through $\nabla_\theta \log \pi_\theta$ using PPO (see \ref{actor_loss}, \ref{critic_loss}), avoiding non-differentiable sampling.  
%(vi) The GCN update in Eq.~\eqref{eq:gcn} is an affine transformation followed by ReLU, hence piecewise-linear and differentiable almost everywhere.  
%(vii) Mean pooling and residual additions are linear and preserve differentiability.

%By closure of (sub)differentiability under composition, the overall mapping from inputs to policy logits and state values is differentiable almost everywhere.  


+

\subsection{Training}


We train the model end-to-end using MAPPO ~\cite{mappo} under CTDE (see Algorithm \ref{alg:plato}). The policy is parameterized by $\theta$ and the centralized critic by $\phi$. During training, agents collect trajectories through interaction with the environment. The pointer actor is updated via the clipped PPO objective,
\begin{equation}
\mathcal{L}_{\pi_i} =
\frac{1}{|\mathcal{B}|}\sum_{j \in \mathcal{B}}
\min\!\left(r_j^i\,\hat{A}_j,\;
\mathrm{clip}\!\left(r_j^i,\,1-\epsilon,\,1+\epsilon\right)\hat{A}_j\right)
- \beta_H\, H(\pi_\theta),
\end{equation}
where
\begin{equation}
r_j^i=\exp\!\big(\log \pi_\theta(a_j|s_j)-\log \pi_{\theta^{\mathrm{old}}}(a_j|s_j)\big).
\end{equation}
Here $\hat{A}_j$ is the generalized advantage estimate \cite{gae}, $\epsilon$ is the clipping threshold, and $\beta_H$ weights the policy entropy $H(\pi_\theta)$, controlling exploration. Our loss is  an average over mini-batches, $\mathcal{B}$. 

The critic estimates $V_\phi(s_t)$ from the global graph. We use MSE, with the PPO clipped value formulation~\cite{ppo}: 

\begin{equation}
\mathcal{L}_V=
\frac{1}{2|\mathcal{B}|}\sum_{j \in \mathcal{B}}
\max\!\left(\left(V_\phi^j-\hat{R}_j\right)^2,\;
\left(V_\phi^{\mathrm{clip},j}-\hat{R}_j\right)^2\right),
\end{equation}
where $V^{clip}$ is the PPO clipped formulation of MSE \cite{ppo}, $\hat{R}_j$ is the empirical return from GAE and $\epsilon_V$ is the value clipping threshold. $V^{clip}$ is calculated as,
\begin{equation}
V_\phi^{\mathrm{clip},j}=V_\phi^{\mathrm{old},j}+\mathrm{clip}\!\left(V_\phi^j-V_\phi^{\mathrm{old},j},-\epsilon_V,\epsilon_V\right).
\end{equation}

\begin{equation}\label{eq:key-integrator-eq}
k^t_x = \mathrm{MLP}_k\left (\mathrm{MLP}_x(o^t_x) + \mathbf{W}_c \times q^t \right ), \quad 
\mathbf{K}^t = [k^t_1 \dots k^t_{|\mathbf{o}^t_X|}; k^t_{\textsc{NOOP}}].
\end{equation}
The outer $\textsc{MLP}_k$, is part of the \emph{key integrator} and projects the conditioned \emph{key} to the decoder's hidden dimension.

The key integrator conditions each task key on $q^t$ (Eq.~\eqref{eq:key-integrator-eq}), making task selection explicitly dependent on the current agent composition under churn.

We create the \emph{key}, $k^t_x$, for a task, $x$, by embedding $o^t_x$ into a latent space using a $\mathrm{MLP}_x$. Then we use a \emph{key-integration} technique inspired by modulation-based feature fusion \cite{perez2018film} to condition each \emph{key} on the \emph{query}, 



\subsection{GNN Critic} \label{critic}

The centralized critic estimates the state value $V_\phi(\text{State}^t)$ under CTDE.
To represent $\text{State}^t$ when the numbers of agents and tasks vary over time, we construct a \textbf{global bipartite graph} $\mathcal{G}^t$ (Fig.~\ref{fig:global_graph}).
The graph contains two node types: agent nodes and task nodes.
We use a bipartite structure because agent entities and task entities have different semantics and feature spaces, and the only relations required for value estimation in our domains are \emph{agent--task feasibility} relations.


\[
\mathcal{G}^t = (\mathcal{X}, \mathcal{N}, \mathcal{E
}),
\]
which encodes the state, $\text{State}^t$, at time $t$, where 
\begin{itemize}
\item $\mathcal{X}^t \in \mathbb{R}^{|X|^t\times f_X}$ are \emph{task nodes} and contain $f_X$ many features, describing each task at time $t$.
\item $\mathcal{N}^t \in \mathbb{R}^{|N|^t\times f_N}$ are \emph{agent nodes} and contain $f_N$ many features, describing each agent at time $t$. 
%\item $\mathcal{V} = \mathcal{A} \cup \mathcal{T}$ contains agent nodes and task nodes,  
\item $\mathcal{E}$ includes undirected edges between all agent-task pairs which have an action, $\{\langle n,x\rangle | n\in \mathcal{N} \text{ and }x\in \mathcal{X}\}$.  
%\item $\mathbf{X} \in \mathbb{R}^{|\mathcal{V}| \times d_x}$ holds the initial node features derived from agent observations and task attributes.  
\end{itemize}

\begin{figure}
  \centering
  \includegraphics[width=0.6\linewidth]{figs/graph_revised.pdf}
\caption{\small This global graph represents the environment state for $i$ agents and $j$ tasks.
Edges encode agents ability to act on tasks.}
\label{fig:global_graph}
\end{figure}

We build a critic network on a graph convolutional neural network (GCN) \cite{kipf2016semi} which propagates  information between nodes (agents and tasks) by \textbf{message passing}. Before we use a GCN, we employ \textbf{MLPs} to bring $\mathcal{X}^t$ and $\mathcal{N}^t$ into the same space,
\begin{equation}
\label{eq:node-embedding}
\mathbf{h}_0^t = \text{Concat}\left [\text{MLP}_{\mathcal{N}}\left ( \mathcal{N}^t \right ), \text{MLP}_\mathcal{X}\left(\mathcal{X}^t \right ) \right ]\quad \mathbf{h}^t_0\in\mathbb{R}^{|\mathcal{G}^t| f_h},
\end{equation}
where $\mathbf{h}_0$ is the embedding of all nodes in $\mathcal{G}^t$, and $f_h$ is the hidden dim. Now, with fixed size features, we perform message passing, 
\begin{equation}
    \label{eq:message-passing}
    \mathbf{h}_1 = \mathrm{ReLU}\left (\frac{\mathbf{h}_0 W_{l}}{\sqrt{|N| \cdot |X|}} \right ) + \mathbf{h}_0,
\end{equation}
where we add $\mathbf{h}_0$ back in as a residual. We use two layers  (replacing $h_0$ with $h_{l-1}$ for layer $l$) to allow information to propagate from agent to agent and task to task through the other.

We map this graph to a scalar value estimate through mean pooling over nodes and a MLP$_v$ over pooled features,
\begin{equation}
\label{eq:value-pooling}
V(\text{State}^t) = MLP_v\left ( \frac{1}{|\mathcal{X}|+|\mathcal{N}|} \sum_{i=1}^{|\mathcal{X}|+|\mathcal{N}|} h^t_{2,i} \right ).
\end{equation}

\begin{algorithm}
\caption{\textsc{PLATO}}
\label{alg:plato}
\scriptsize
\begin{algorithmic}[1]
\State \textbf{Inputs:} env $e$, horizon $T$, actor $\pi_\theta$, critic $V_\phi$, initial observation $\mathbf{O}^0$
\For{$t=1\ldots T$} 
  \State $a^t_i\sim \textsc{PointerActor}(\mathbf{O}^t; \theta) \quad \forall i \in N$
  \State $\mathbf{O}^t,\text{State}^t,r^t\gets e(\mathbf{a}^t)$
  \State $\hat V^t \gets \textsc{GNNCritic}(\text{State}^t;\phi)$;\; store $(\cdot)$
  \State  compute GAE $\hat A^t$;\; update $\theta$ by PPO-clip;\; update $\phi$ by MSE$(\hat V^t,\hat R^t)$
\EndFor
\Statex

\Procedure{\textsc{PointerActor}}{$\mathbf{O}^t$}
  \State $\mathbf{o}_n^t,\mathbf{o}_X^t\gets \textsc{Preprocessor}(\mathbf{O}^t)$ 
  \Comment{Agent Encoding}
  \State $\mathbf{s}^t\!\gets\![\mu,\sigma^2,\min,\max](\mathbf{o}^t_{N})$
  \State $q^t \gets \mathrm{LSTM}\left (\textsc{MLP}_s(d^t),q^{t-1} \right )$
  \Comment{Task Encoding}
  \State $\mathbf{K}^t \gets \mathrm{MLP}_k\left (\mathrm{MLP}_x(o) + \mathbf{W}_c \times q^t \right ) \quad \forall o \in o^t_X \cup \textsc{NO-OP}$
  \State $u_i\!\gets\!\mathbf{v}^\top\tanh(\mathbf{W}_k \times k^t_x+\mathbf{W}_q\times q^t) \quad \forall k_x^t \in \mathbf{K}^t$ 
  \Comment{Pointer Decoding}
  \State  \textbf{return} $\mathrm{Cat}(\mathrm{softmax}([u_i]))$
\EndProcedure
\Statex
\Procedure{\textsc{GNNCritic}}{$\text{State}_t$} 
  \State form $\mathcal{G}^t=\langle\mathcal{X}^t,\mathcal{N}^t,\mathcal{E}^t\rangle$
  \State $\mathbf{h}_0^t \gets \text{Concat}\left [\text{MLP}_{\mathcal{N}}\left ( \mathcal{N}^t \right ), \text{MLP}_\mathcal{X}\left(\mathcal{X}^t \right ) \right ]$
  \State $\mathbf{h}^t_l \gets \textsc{GCN}(\mathbf{h}_{l-1}, \mathcal{E}) \quad \text{for each layer }l$
  %\!\gets\!\mathrm{ReLU}(\tilde{\mathbf{D}}^{-\frac12}\tilde{\mathbf{A}}\tilde{\mathbf{D}}^{-\frac12}\mathrm{ReLU}(\tilde{\mathbf{D}}^{-\frac12}\tilde{\mathbf{A}}\tilde{\mathbf{D}}^{-\frac12}\mathbf{e}_g\mathbf{W}^{(1)})\mathbf{W}^{(2)})$
  \State $\mathbf{M}^{(L)}\!\gets\!\frac{1}{|\mathcal{V}|}\sum_i(\mathbf{H}^{(2)}+\mathbf{e}_g)_i$;\;
  \State \textbf{return} $V=\mathbf{W}_v\,\mathrm{MLP}_v(\mathbf{M}^{(L)})+b_v$
\EndProcedure
\end{algorithmic}
\end{algorithm}


